MedFilter: Improving Extraction of Task-relevant Utterances from Doctor-Patient Conversations through Integration of Discourse Structure and Ontological Knowledge

Information extraction from conversational data is particularly challenging because the task-centric nature of conversation allows for effective communication of implicit information by humans, but is challenging for machines. The challenges may differ between utterances depending on the role of the speaker within the conversation, especially when relevant expertise is distributed asymmetrically across roles. Further, the challenges may also increase over the conversation as more shared context is built up through information communicated implicitly earlier in the dialogue. In this paper, we propose the novel modeling approach MedFilter, which addresses these insights in order to increase performance at identifying and categorizing task-relevant utterances, and in so doing, positively impacts performance at a downstream information extraction task. We evaluate this approach on a corpus of nearly 7,000 doctor-patient conversations where MedFilter is used to identify medically relevant contributions to the discussion (achieving a 10% improvement over SOTA baselines in terms of area under the PR curve). Identifying task-relevant utterances benefits downstream medical processing, achieving improvements of 15%, 105%, and 23% respectively for the extraction of symptoms, medications, and complaints.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> sections/data.tex <==
\subsection{Corpus Description}
\label{sec:data}

Our dataset comprises of 6,862 de-identified real doctor-patient conversations. 
% All the transcripts are manually transcribed and annotated by the experts. 
The conversations have an average of 225 utterances of doctor and patient and occasionally from nurses, caregivers, and other attendees as well. 
% \todo{Add data distribution in the appendix}
% The sentences in the transcript are grounded to the audio with the timestamp of their first and last words. 
Individual utterances are annotated with medical class tags deemed relevant by the expert annotators. Given the informal nature of conversations in the corpus, many of the utterances within them are irrelevant for the downstream clinical tasks\footnote{Example (details changed) conversation shown in Table~\ref{tab:conv} in the Appendix.}.

The annotation guidelines were developed by a team of professional medical scribes and NLP experts. The annotators were asked to identify medically relevant utterances in a given conversation and assign a corresponding tag to each utterance. For instance, labeling an utterance as \textit{symptom}, \textit{previous medical history}, \textit{diagnosis} etc. 

In this paper, we leverage these labels to train \method{} on the task of utterance classification and constrain ourselves to three categories, namely, \textit{symptoms}, \textit{complaints}, and \textit{medications}, where \textit{medications} include past/current medications taken by the patient and prescriptions given by the doctor. However, our approach can be easily generalized for capturing other aspects such as \textit{previous medical history}, \textit{diagnosis}, and \textit{assessments} as well. 
We set aside a random sample of 627 and 592 conversations for validation and testing respectively.
% In addition to identifying the type of each utterance, annotators also provide a class label to them from a predefined set. For symptoms, guidelines include around 150 classes of the form \textit{<Body System>: <Issue>} (e.g. Cardiovascular: Palpitations). Given the small size of the training data, instead of predicting given symptom classes in our extraction based evaluation experiments, we predict the body system with which they are associated. Similarly, there is a predefined set of classes defined for medications. We manually link each medication label to its corresponding UMLS~\cite{umls} concept and group them using hierarchies from 
% %SNOMED CT \cite{snomed} and 
% NCI Thesaurus \cite{nci} 
% %respectively
% . This alleviates label-sparsity and reduces label count to $14$ for symptoms and $32$ for medications.\footnote{Please refer to the Appendix for the final list of labels.} We set aside a random sample of around 627 and 592 conversations for validation and testing respectively.
% For the experiments in this paper, we constrain ourselves to three of these medical categories, namely, \textit{symptoms} (concerns), \textit{complaints} (identified issues), and \textit{medications} (prescribed solutions), where \textit{medications} include past/current medications taken by the patient and prescriptions given by the doctor. 
% These three topics form a major part of the medical information patient cares about, they occur in almost all conversations thus allowing us to use the full corpus for our experimentation, and these abstract concepts generalize well to other task domains like customer-service chats.
% However, our proposed approach can be easily extended to identify other types of utterances as well. 
% \todo{Give an example conversation}
% \method{} takes in these transcribed conversations as input
% %which are obtained from speech diarization \cite{speech_diar1,speech_diar2} and recognition \cite{med_speech_recog} systems. 
% to identify medically relevant utterances and their respective categories.
%The transcripts are de-identified with [\url{de-identified}] tags. Individual utterances are annotated with medical class tags deemed relevant by the expert annotators (as shown in Table~\ref{tab:labels}). 
%\noindent
%\textbf{Symptom Annotations} are created using the template \textit{<Body System>: <Issue>}. Raw annotations contain $100$ classes and are reduced down to $14$ in this work to represent the \textit{<Body System>} the symptom affects and to alleviate label sparsity. The individual labels are mentioned in Table~\ref{tab:sym}.
%\noindent
%\textbf{Medication and Chief Complaint} labels are reduced using their corresponding hierarchies in UMLS. UMLS metatheasurus contains hierarchical relations taken from different formal medical vocabularies like SNOMED-CT, NCI, MTH etc. We map chief-complaints and medications to their corresponding concepts in UMLS using QuickUMLS (CITATION) and take the first four nodes in the hierarchy generated from SNOMED-CT and NCI respectively and then combine some of them to reduce label sparsity. For medications that do not have a corresponding NCI hierarchy, we map them with the hierarchy of their tradename. This reduces the labels from $111$ to $10$ for complaints (Table~\ref{tab:comp}) and $1111$ to $33$ for assessments (Table~\ref{tab:med}).

==> sections/extractor.tex <==
\subsection{Medical Footprint Extractor}
\label{sec:footprint_extractor}

In this section, we describe the second component of \method{}. Here, we further process the extracted utterances to identify overall symptoms, complaints and medications discussed in the conversation. We claim that instead of processing the entire conversation for capturing different medical information, our hierarchical approach provides an advantage as it shares parameters across different tasks. This is essential in medical domain where there is a dearth of training data \cite{med_data_scarcity} due to privacy issues and sensitive nature of the data. Also, our approach makes the neural model more interpretable which are criticized for being black-box \cite{black_box_nn}. Below we present the models which we use for capturing different medical information. 

\textbf{Extractor Architecture:}
For extracting symptoms, we constraint ourselves to the utterances marked with the same label by utterance classifier. The problem is modeled as a multi-label classification task with 14 predefined classes (listed in supplementary). Each class indicate the body system being affected because of the underlying disease. Similar to utterance classifier, we first encode all utterances marked as symptoms $\{\hat{u}_1, \hat{u}_2, .., \hat{u}_k\}$ using a BERT-based encoder followed by \texttt{MEAN} pooling. This gives a representation $\bm{\hat{h}}_i$ for each utterance. Then, for capturing inter-relationships between difference utterances, we utilize self-attention \cite{self_attention,transformer} and obtain an updated representation $\bm{\hat{H}}^{\mathtt{self}}$ for all utterance given as,
 \[
\bm{\hat{H}}^{\mathtt{self}} = \mathrm{softmax}\left( \dfrac{\bm{Q}\bm{K}^T}{\sqrt{d}}\bm{V}\right),
\] 
\[
\text{where} \ \ \bm{Q} = \bm{W}_Q \bm{\hat{H}}; \bm{K} = \bm{W}_K \bm{\hat{H}}; \bm{V} = \bm{W}_V \bm{\hat{H}}; \ \ \bm{\hat{H}} = [\bm{\hat{h}_1}, \bm{\hat{h}}_2, ..., \bm{\hat{h}}_k]. 
\]
Here,  $\bm{W}_Q, \bm{W}_K, \bm{W}_V \in \real{d \times d}$ are model parameters which are learned during training. Now, for getting a representation for the entire conversation $\bm{\hat{h}}'$ and pruning out irrelevant utterances, we use \newcite{bahdanau_att}'s attention defined as,
\[
\bm{\hat{h}}' = \sum_{i=1}^{k}\alpha_i \bm{\hat{h}}_i^{\mathtt{self}},
\]
\[
\text{where} \ \alpha_i = \dfrac{\mathrm{exp} (\bm{u}_i^{T} \bm{c})}{\sum_j{\mathrm{exp} (\bm{u}_j^{T} \bm{c})}}, \ \ \bm{u}_i = \mathrm{tanh}(\bm{W}\bm{\hat{h}}_i^{\mathtt{self}} + \bm{b}).
\]

Finally,  $\bm{\hat{h}}' $ is fed to a linear classifier followed by a sigmoid for multi-label classification as defined in the previous section. A similar model is utilized for identifying the chief complaints and medications in the conversations. The set of predefined labels for both the tasks are included in the supplementary. Since medication comprises of a large number of categories as it ranges from pharmaceutical drugs and food products to physical exercises, apart from the above proposed model, we also explore an information extraction based approach. For that we use, recently proposed medical entity-linker \cite{qumls,scispacy} for identifying the medications in the identified utterances. We explore both the approaches in Section \ref{sec:results}.

%Doctor-patient conversations observe discussion about different body systems. The patient might bring up existing symptoms they are facing, whereas at other times the doctor might have to extract this information from the patient to make informed decisions about the underlying disease or complaint. Here, we attempt to extract these symptoms automatically, so the doctor would not have to go through the conversation themselves. We model the problem of symptom extraction as a multi-label task with 15 possible labels (shown in Appendix) for each conversation. 
%Our model is a BiLSTM with attention. Each utterance in the conversation is passed through the embedding layer and a BiLSTM layer to obtain a contextualized representation.
%\begin{equation}
%\begin{split}
%    h_i & = BiLSTM(e(s_i), h_{i-1}) \\
%    \mathbf{H_i} & = \{h_1, h_2, ..., h_n\}
%\end{split}
%\end{equation}
%where $e()$ is the embedding function.
%The final state of the BiLSTM is re-weighted using attention calculated as shown in Equation 1.
%\begin{equation}
%\begin{split}
%    h_{final} & = [h_0; h_{n-1}] \\
%    \textbf{S} & = \mathbf{H_i}  h_{final} \\
%    \textbf{A} & = softmax(\textbf{S}) \\
%    h'_{final} & = \mathbf{H_i^T}\mathbf{A}
%\end{split}
%\end{equation}
%This allows our model to pay attention to important utterances in the conversation to extract symptom information. We pass $h'_{final}$ through a linear classifier and a sigmoid layer to get logits for each possible symptom label.

%\textbf{Chief Complaint Classification}
%We implement a similar BiLSTM-Attention model to classify each conversation with a chief complaint. Being a multi-class problem, we switch the sigmoid layer in the symptom extractor with a softmax layer to get the most probable complaint.

%\textbf{Medication Extraction}


%
%For medication extraction, apart for the architecture used for symptom and complaint analysis, we also explore an extraction based approach. 
%
% as a classification problem as we did not find an exhaustive list of categories, medications can be divided into. Medications are not necessarily constraint to medicines as a doctor may prescribe behavioral changes or food products thus expanding the scope of possible categories.
%In this work, we do not propose a state-of-the-art method for medication extraction but merely use this task to evaluate the performance of our summarization model. We use QuickUMLS entity-linker to extract medication names from the conversation and tie them back to UMLS.


==> sections/introduction.tex <==

\section{Introduction}
\label{sec:introduction}
A general class of problems in NLP is to convert the information discussed in conversations into a structured format.
% , e.g. summarizing meetings, or creating Electronic Health Record (EHR) entries from doctor-patient conversations. 
Several of the challenges in this direction stem from the fact that human-to-human conversations lack clear boundaries and structure. 
Moreover, neighbouring utterances in the conversation may seem drastically different in terms of topics they discuss~\cite{waitzkin1989critical}.
% its organization can never be top-down with a singular focus, in part because more than one person's perspective is involved.
% This is especially true when the dialogue is goal oriented and there is an asymmetry between the speakers in terms of knowledge or authority. For example, in expert-lay conversations like customer-service chats or doctor-patient interactions, the layperson voices their concerns, whereas the expert identifies the underlying issue and prescribes solutions.
For example, in doctor-patient conversations, the doctor may jump from question about a symptom to another for providing initial assessment about a condition then back to asking about symptoms. 
This makes topic segmentation fairly difficult thus exacerbating the difficulties of summarization and information extraction~\cite{lacson2006automatic}.

% A significant amount of time in a medical practitioner's day is spent in summarizing their meetings with the patient and converting them in a format suitable for storage (Electronic Health Records) and future querying. While automatic scribes could aid in providing written records of the discussion, these conversations are usually long and difficult to comprehend due to disfluencies and redundancies. This burden often leads to doctor burnout they might have to complete the documentation outside of work hours.
% Information extraction from dialogues is a challenging task as 

% The field of text summarization has progressed a lot over the past 40 years~\cite{chatbot1,chatbot2}.
% However, work related to the summarization of discussion data has been less prevalent. Arguably, conversation summarization is more challenging since
% its organization can never be top-down with a singular focus, in part because more than one person's perspective is involved.
% This is especially true when the dialogue is goal oriented and there is an asymmetry between the speakers in terms of knowledge or authority. For example, in expert-lay conversations like customer-service chats or doctor-patient interactions, the layperson voices their concerns, whereas the expert identifies the underlying issue and prescribes solutions.

% \newcite{med_scribe_challenge} discuss multiple challenges associated with creating a digital scribe, that would automatically convert the audio from a doctor-patient encounter to a structured summary useful for future decision making. 
% Several of the challenges in extracting relevant information from dialogue stem from the fact that human-to-human conversations lack clear boundaries and structure.
% due to the nature of human-to-human conversations. 

Goal-oriented expert-lay dialogue like customer-service chats or doctor-patient interactions are a subclass of conversations that are often mapped to well-defined schema to concisely maintain the logical structure of the discussion for future use~\cite{topic_summ1,topic_summ2}. This schema encodes topics like the concerns voiced by the layperson (e.g. symptoms), the underlying issue identified by the expert (e.g. complaint) and the prescribed solutions (e.g. medications). The participants make unequal contributions to different parts of the schema due to the inherent asymmetry between them in terms of knowledge and authority. 

% successful interaction would witness the layperson voicing their concerns (e.g. symptoms), and the expert trying to identify the underlying issue (e.g. complaint) and prescribe solutions (e.g. medications).
% and contain an inherent asymmetry between speakers in terms of knowledge and authority. This results in the participants making unequal contributions to different parts of the required output schema (as a function of their knowledge).
% However, the intentions of the speakers in expert-lay conversation like doctor-patient interactions or customer-service chats often act as logical steps (or themes) in the path (or schema) which is followed to reach the goal of the encounter~\cite{topic_summ1,topic_summ2}. 
% For example, a successful interaction would witness the layperson voicing their concerns (e.g. symptoms), and the expert trying to identify the underlying issue (e.g. complaint) and prescribe solutions (e.g. medications). Such a structure provides additional signal that can be leveraged to improve downstream processing. 

In this work, we propose \method{}, a novel approach to automatically identify the dialogue utterances that contain information essential to populate this schema. 
% We make the following contributions: 
% \noindent\textbf{(i)}
% We propose \method{}, a novel approach to identify the parts of the conversation that contain information essential to populate parts of this schema.
We focus on the use-case of extracting medically relevant utterances from doctor-patient conversations and categorizing them into the medical topics/categories they describe. 

% According to recent studies~\cite{rena2018burnout,wachter2018combat,arndt2017tethered}, $50\%$ of the physicians in the United States of America suffer from burnout~\cite{burnout_ehr} due to the overhead of administrative tasks such as EHR documentation. 
% % Furthermore, as the EHR documentation happens post-conversation, its quality is limited by physician's recall power which can have severe consequences \cite{ehr_errors}.
% Therefore, automatically identifying utterances that discuss these topics holds the potential to facilitate faster downstream processing of medical conversations. 
\begin{figure*}
	\centering
	\includegraphics[width=0.8\textwidth]{./Images/overview_sopan_pdf}
	\captionsetup{font=small,labelfont=small}
	\caption{\label{fig:workflow} Overview of \method{}. \method{} first encodes each utterance of the given clinical conversation using a BERT-based encoder. The obtained utterance embedding is concatenated with a variety of side information extracted from the conversation. This is then fed to a hierarchical MS-BiLSTM architecture for classification. Refer to Section \ref{sec:utt_class} for more details.}
	\vspace{-0.3cm}
\end{figure*}
Performing automatic topic-segmentation in doctor-patient dialogues has substantial practical impact in the medical profession \cite{naacl18_med_scribe,med_scribe_challenge}, especially when those topics map to different categories in the clinical note~\cite{soap_note} that is composed, currently manually, for each encounter to document a patient's progress.

\method{} (Section~\ref{sec:utt_class}) leverages side-information like discourse structure and domain knowledge to perform this segmentation.
To explicitly model the separate roles taken up by each speaker, we introduce MS-BiLSTM which learns speaker-specific context representations. \method{} also benefits from the incorporation of a generalizable hierarchical loss that jointly learns the coarse-grained task of predicting medical relevance to improve fine-grained topic-based utterance classification (Figure~\ref{fig:workflow}).

We measure \method{}'s performance (Sections~\ref{sec:setup}, \ref{sec:results}) on
% For the experiments in this paper, we constrain ourselves to 
% three of these medical categories, namely, 
\textit{symptoms}, \textit{complaints}, and \textit{medications}, the three categories of interaction that are a part of every office visit 
% form a major part of the medical information patient cares about, occur in almost all conversations thus allowing us to use the full corpus for our experimentation, 
and most closely generalize to other domains like customer-service chats.

To gauge the benefits of this topic-based classification on downstream tasks of medication and symptom extraction (Figure~\ref{fig:main_fig}), we use our system as a pre-processing step to filter out utterances irrelevant to the tasks (Section~\ref{sec:footprint_extractor}). 
% For example, we prune all non-symptomatic utterances as predicted by \method{} before passing through the symptom extractor. 
% prowess on reducing the amount further evaluate our system's prowess as a pre-processing step in the downstream tasks of medication and symptom extraction. 
We provide a detailed analysis of the contributions of domain knowledge and discourse information and conclude with a systematic investigation of the errors made by \method{} (Section~\ref{sec:discussion}).
% tasks in a goal-oriented conversation and categorizes them into the user intent the describe.

% medically relevant utterances and classify them into the medical topics/categories they describe (Section ~\ref{sec:utt_class})
% Correctly identifying the information that forms each 
% Expert-lay conversations like doctor-patient interactions or customer-service chats are usually goal-oriented, where the layperson voices their concerns (e.g. symptoms), and the expert tries to identify the underlying issue (e.g. complaint) and prescribe solutions (e.g. medications). Often, these discussed topics (symptoms, complaints, medications) map to the attributes of a logical schema of the discussion (e.g. Electronic Health Records (EHRs)) which is composed, currently manually, for the ease of future querying and decision making.
% Extracting such a logical structure is particularly useful when the dialogue is goal-oriented. For example, in expert-lay conversations like customer-service chats or doctor-patient interactions, where the layperson voices their concerns, whereas the expert identifies the underlying issue and prescribes solutions, sorting utterances that discuss the aforementioned topics would also allow downstream processing to focus on information relevant for their task thus improving the signal-to-noise ratio of the input.
% \newcite{med_scribe_challenge} discuss multiple challenges associated with creating a digital scribe for doctor-patient conversations. 
% These challenges can be generalized to other expert-lay dialogue that incorporate domain knowledge. In this work, we try to extract topics at the granularity of medical categories like symptom/ complaint/ medication etc to assist downstream medical processing.
% Nevertheless, conversation summarization is an area with substantial potential practical impact \cite{conv_summ1,conv_summ2}, especially in the medical profession \cite{naacl18_med_scribe,med_scribe_challenge}, where the work of conducting doctor's visits is done through conversation, and a written summary of that encounter is required to be composed for future reference. These summaries usually adhere to specific formats (e.g. Electronic Health Records (EHRs)) for the ease of querying in future.
% According to recent studies~\cite{rena2018burnout,wachter2018combat,arndt2017tethered}, $50\%$ of the physicians in the United States of America suffer from burnout~\cite{burnout_ehr} due to the overhead of administrative tasks such as EHR documentation. 
% % Furthermore, as the EHR documentation happens post-conversation, its quality is limited by physician's recall power which can have severe consequences \cite{ehr_errors}.
% Therefore, automatically identifying utterances that discuss these topics holds the potential to facilitate faster downstream processing of medical conversations. 

% To this end,
% \todo{Tweak intro to talk more about works where side-info helps?}
% \newcite{naacl18_med_scribe} present an abstract prototype design for a virtual scribe to create such summaries and posit that extracting medically relevant utterances from conversations is an essential component in the automated medical scribe pipeline.
% Inline with the intuition of ~\newcite{mayfield2013recognizing}, utterance-level categorization (content selection) can also be helpful as a pre-processing step to allow downstream tasks such as symptom extraction~\cite{acl19_symptom}, symptom summarization~\cite{liu2019topicsumm}, or regimen extraction \cite{diagnosis_detection} to focus on relevant portions of the conversations. 
% Furthermore, it can even be employed as a standalone system to reduce the amount of text the doctors are required to process everyday.

% Apart from assisting summarization, \method{} can also be helpful as a pre-processing step to allow downstream tasks such as symptom extraction~\cite{acl19_symptom},
% % symptom summarization~\cite{liu2019topicsumm}, 
% or regimen extraction \cite{diagnosis_detection} to focus on relevant portions of the conversations. 
% Furthermore, it can even be employed as a standalone system to reduce the amount of text the doctors are required to process everyday.

\noindent Our contributions can be summarized as follows\todo{Is this required}.
{\begin{enumerate}
[itemsep=2pt,parsep=0pt,partopsep=0pt,leftmargin=*,topsep=0.2pt]
    \item We propose \method{}, a neural network-based method for automatic tagging of utterances in doctor-patient conversations based upon the information they provide. 
    \item We make 
    makes principled use of side information and utilizes speaker-specific context and a hierarchical loss function to obtain state-of-the-art results on the task. 
    \item We evaluate the benefits of leveraging medical topic-based utterance classification as a pre-processing step for downstream extraction tasks.
\end{enumerate}}
\begin{figure}[h]
    \vspace{-0.3cm}
	\centering
	\includegraphics[width=0.9\linewidth]{./Images/main_fig}
	\captionsetup{font=small,labelfont=small}
	\caption{\label{fig:main_fig}\method{} as a part of the medical summarization and extraction pipeline.}
	\vspace{-0.3cm}
\end{figure}




==> sections/overview.tex <==
\section{\method{} Overview}
\label{sec:overview}

In this section, we present a brief overview of \method{}, our proposed method for automating structured summarization of clinical conversations. \method{} takes in a transcribed conversation as input
%which are obtained from speech diarization \cite{speech_diar1,speech_diar2} and recognition \cite{med_speech_recog} systems. 
for identifying clinical footprints, i.e., detecting symptoms, assessment, etc. In this paper, we focus on extracting three such information, namely, symptoms, chief complaint, and medications. However, our method can be easier extended to capture other types of information as well. In general, medical conversations contain multiple utterances and given its informal nature many of them are irrelevant for the downstream clinical tasks. We handle this challenge in \method{} through a two-step hierarchical approach. First, our method identifies utterances which are relevant for identifying particular medical information and prunes out irrelevant utterances. Then, we perform analysis of the subset of utterances for extracting fine-grained categories of symptoms, medications and complaints. The overall architecture of \method{} is shown in Figure \ref{fig:workflow}. 
%Along with identifying different information, \method{} also recognizes interrelationships between them. For instance, symptoms such \textit{cough} and \textit{hemoptysis} can be related with chief complaint \textit{tuberculosis}. 
%This is accomplished by utilizing knowledge sources such as UMLS (Unified Medical Language System) \cite{umls} and WikiData \cite{wikidata}. 
Below we describe both the components in brief.

\begin{enumerate}
    \item \textbf{Utterance Classifier:} For a given transcribed clinical conversation, \method{} classifies each utterance as symptom, chief complaint, medication, or not medically relevant. Each utterance is first encoded using a BERT-based \cite{bert} encoder which is passed to a Recurrent Neural Network (RNN) \cite{lstm} for encoding the context of each utterance. Finally, the obtained representation is passed to a feedforward network based classifier for prediction. This component also utilizes hierarchical loss and relevant signals from UMLS knowledge graph for improving on this task. Please refer to Section \ref{sec:utterance_class} for details.
    
    \item \textbf{Medical Footprint Extractor:} Now, based on the type assigned by the previous module, each utterance is further analyzed to identify the specific category of each information. For instance, symptoms are classified as cardiovascular, respiratory, musculoskeletal, etc. Finally, based on all the information is extracted and UMLS knowledge graph, a summary is generated for the entire conversation in the form of a graph. More details are provided in Section \ref{sec:footprint_extractor}.
\end{enumerate}

%symptoms, assessments, and complaint mentioning utterances from conversations as a hierarchical sequence-labeling task. This would allow us to provide doctors with direct utterance-level evidence of the presence of these attributes in the conversation.

%Since our data has labels for whether the utterance is medically relevant, does it talk about a symptom/assessment/complaint and which category of symptoms it belongs to, we can create a model that leverages these hierarchical labels to learn representations beneficial for each step and use them to further inform the next level of classification. 

%We train this hierarchical model end-to-end with a multi-task learning framework jointly optimizing the losses at each level. We will explain the components of our model in the next few sections.

